$\mathscr Q$-Sets and Friends: Categorical Constructions and Categorical Properties

This work mainly concerns the -- here introduced -- category of $\mathscr Q$-sets and functional morphisms, where $\mathscr Q$ is a commutative semicartesian quantale. We describe, in detail, the limits and colimits of this complete and cocomplete category and prove that it has a classifier for regular subobjects. Moreover, we prove that it is $\kappa^+$-locally presentable category, where $\kappa=max\{|\mathscr Q|, \aleph_0)\}$ and describe a hierarchy of semicartesian monoidal closed structures in this category. Finally, we discuss the issue of 'change of basis' induced by appropriate morphisms between the parametrizing quantales involved in the definition of $\mathscr Q$-sets. In a future work we will address such questions in the full subcategory given by all Scott-complete $\mathscr Q$-sets

==> constructions-section/classifier.tex <==
migrou para subsecao em  arquivo unificado limcolimetc

==> constructions-section/restos.tex <==
\section{Colimits}

\begin{example}[Initial Object]
    The empty set is -- vacuously -- a \(\quantale Q\)-set, and since
    morphisms are functions, it also happens to be the initial object.
\end{example}


\begin{prop}[Initial object]
    The terminal object is \(\bot = (\varnothing,\varnothing)\)
\end{prop}
\begin{proof}
    This is a \(\quantale Q\)-set by vacuity. The empty function is a morphism
    again by vacuity, and it obviously must be the initial object, as morphisms
    are -- in particular -- functions as well.
\end{proof}

\begin{prop}[Non-empty coproducts]
    The coproduct of \(\quantale Q\)-sets \((X_i)_{i \in I}\) is:
    \begin{align*}
        \coprod_{i \in I} X_i&=(\coprod_{i \in I}|X_i|, \delta)\\
        \delta((x,i),(y,i))  &= \begin{cases}
            \delta_i(x,y), &i = j\\
            \bot,          &i\not= j. 
        \end{cases}
    \end{align*}
\end{prop}
\begin{proof}[Proof: It is a \(\quantale Q\)-set]
    Suppose that \(i\neq j \neq k \neq i\). Without loss of generality:
    \begin{align*}
        \tag{\(\delta\) is symmetric}
        \delta((x,i),(y,i))&=\delta_i(x,y)\\
        &=\delta_i(y,x)\\
        &=\delta((y,i),(x,i))\\
        \\
        \delta((x,i),(y,j))&=\bot\\
        &=\delta((y,j),(x,i))\\
        \\
        \tag{extensionality}
        \delta((x,i),(y,i))\tensor E(x,i) &= \delta_i(x,y) \tensor Ex\\
        &= \delta_i(x,y)\\
        &= \delta((x,i),(y,i))\\
        \\
        \delta((x,i),(y,j)\tensor E(x,i) &= \bot\tensor Ex\\
        &= \bot\\
        &= \delta((x,i),(y,j))\\
        \\
        \tag{triangular inequality}
        \delta((x,i),(y,i))\tensor \delta((y,i),(z,i)) &= \delta_i(x,y)\tensor \delta_i(y,z)\\
        &\leq\delta_i(x,z)\\
        &=\delta((x,i),(z,i))\\
        \\
        \delta((x,i),(y,j)\tensor\delta((y,j),(z,j))&=\bot\tensor\delta((y,j),(z,j)\\
        &= \bot\\
        &\leq \delta((x,i),(z,j))\\
        \\
        \delta((x,i),(y,j)\tensor \delta((y,j),(z,k)) &= \bot\tensor \bot\\
        &= \bot\\
        &\leq \delta((x,i),(z,k))
    \end{align*}
\end{proof}
\begin{proof}[Proof: Coprojections]
    \begin{align*}
        \coproj_i: X_i\to& \coprod_{i \in I} X_i \\
        \coproj_i(x_i)   &= (x_i,i)
    \end{align*}
    By construction those are obviously morphims.
\end{proof}
\begin{proof}[Proof: Universality]
    Let \(f_i:X_i\to A\) a family of morphisms. We define:
    \begin{align*}
        h: \coprod_{i \in I} X_i &\to A\\
        h(x,i)                   & =  f_i(x)
    \end{align*}
    Then \(h\) satisfies the universal property:
    \begin{align*}
        f_i\circ\coproj_i(x,i)=f_i(x)&=h(x,i)\\
        f_i\circ\coproj_i&=h
    \end{align*}
\end{proof}


\begin{example}
    Given a nonempty index set \(I\), we have a 
    \(\quantale Q\)-set \(\coprod_{i\in I}\top\), given by
    \[
        \delta((e, i), (e', i')) = \begin{cases}
            e\wedge e', &\text{if} ~ i = i';\\
            \bot,       &\text{otherwise}.
        \end{cases}
    \]    
\end{example}

\begin{prop}[Coequalizers]
    For $f,g:(X,\delta) \to (Y,\delta')$, we define the equivalence relation $\sim \ \subseteq |Y|\times |Y|$ as the transitive closure of $f(x)\sim f(x)\sim g(x)\sim g(x)$.

    The coequalizer of $f,g:(X,\delta) \to (Y,\delta')$ is:\\
    \begin{align*}
    \coequalizer (f,g)&=\left(\faktor Y \sim,\delta\right)\\
    \delta(\eqclass{y},\eqclass{y'})&= \bigvee_{\substack{a\sim y\\a'\sim y'}}      
        \delta(a,a') 
    \end{align*}
\end{prop}
\begin{proof}[Proof: \(\quantale Q\)-set]
    \begin{align*}
        \delta(\eqclass{y},\eqclass{y'})
        &=  \bigvee_{\substack{a\sim y\\a'\sim y'}} 
                \delta(a,a')
        =   \bigvee_{\substack{a\sim y\\a'\sim y'}} 
            \delta(a',a)
        \\&=\delta(\eqclass{y'},\eqclass{y})
    \end{align*}
    \begin{align*}
        \delta(\eqclass{y},\eqclass{y'})
        &\geq
            \delta(\eqclass{y},\eqclass{y'})
            \tensor
            \extent\eqclass{y}
        \\&=\delta(\eqclass{y},\eqclass{y'})
            \tensor 
            \bigvee_{\substack{a\sim y\\a'\sim y}}\delta(a',a)
        \\&=\bigvee_{\substack{a\sim y\\a'\sim y'}}\delta(a',a)
                \tensor 
            \bigvee_{a\sim y} Ea 
        \\&\geq
            \bigvee_{\substack{a\sim y\\a'\sim y'}} 
                \delta(a',a)\tensor Ea
        \\&=\bigvee_{\substack{a\sim y\\a'\sim y'}} \delta(a',a)
        \\&=\delta(\eqclass{y},\eqclass{y'})
    \end{align*}
    \begin{align*}
        \delta(\eqclass{y},\eqclass{y'})
        \tensor 
        \delta(\eqclass{y'},\eqclass{y''})
        &=  \bigvee_{\substack{a\sim y\\a'\sim y'}} \delta(a',a) \tensor
            \bigvee_{\substack{b\sim y'\\b'\sim y''}} \delta(b,b')
        \\&=\bigvee_{\substack{a\sim y\\a'\sim y'}}
            \bigvee_{\substack{b\sim y'\\b'\sim y''}}
                \delta(a',a) \tensor \delta(b,b')
        \\&=\bigvee_{\substack{a\sim y\\a'\sim y'}}
            \bigvee_{\substack{b\sim y'\\b'\sim y''}}
                \delta(a',a) \tensor Ea \tensor \delta(b,b')
        \\&=\bigvee_{\substack{a\sim y\\a'\sim y'}}
            \bigvee_{\substack{b\sim y'\\b'\sim y''}}
                \delta(a',a) \tensor 
                \delta(a,b)  \tensor
                \delta(b,b')
        \\&\leq
            \bigvee_{\substack{a\sim y\\a'\sim y'}}
            \bigvee_{\substack{b\sim y'\\b'\sim y''}} 
                \delta(a,b) \tensor \delta(b,b')
        \\&\leq
            \bigvee_{\substack{a\sim y\\a'\sim y'}}
            \bigvee_{\substack{b\sim y'\\b'\sim y''}} 
                \delta(a,b')
        \\&=\bigvee_{\substack{a\sim y\\b'\sim y'}} 
            \delta(a,b')
        \\&=\delta(\eqclass{y},\eqclass{y''})
    \end{align*}
\end{proof}

\begin{prop}[Epimorphisms]
    Epimorphisms are precisely the surjective morphisms. 
    Suppose that $f:X \to Y$ is surjective. Then, 
    $\forall y \in Y: \exists x \in X: f(x)=y$. Let $g,h:Y\to A$. 
    Suppose that $\forall x \in X :g \circ f(x)=h \circ f(x)$. 
    Let $y \in Y$. There is a $x \in X$ such that $f(x)=y$. 
    Then $g(y)=g \circ f(x)=h\circ f(x)=h(y)$.\\
\end{prop}
\begin{proof}
    Take some \(f:X\to Y\) and suppose
    \[
        \exists y_0\in Y:\forall x\in X: f(x)\not = y_0
    \]
    Let \(Y_f=\left(\faktor{(Y\amalg Y)}\sim, \delta\right)\), 
    as generated by 
    \[
        y\in\img f \implies \coproj_l(y) \sim \coproj_r(y)
    \]
    Let $g,h:Y\to Y_f$ as $g(y)=[(y,0)]$ and $h(y)=[(y,1)]$. 
    Then $g\neq h$ but $g \circ f = h \circ f$.
    \zeca{eu não entendi e nem sei se é verdade}.
    \caio{vou detalhar mais.}

    
    
\end{proof}

\section{Generators and Classifier}

The main goal of this section is to establish that the category \(\quantale Q\)-sets has a (almost trivial) classifier for the regular subobjects.

\hugo{Import from Caio's files}

\begin{prop}[Separating Family]
    For each \(e \in \extent\quantale Q\) (ie. the terminal object) we 
    can consider the singleton set formed by \(e\) with a natural 
    \(\quantale Q\)-set structure as inherited from \(\extent\quantale Q\).
    
    In fact, the set of such \(\quantale Q\)-sets is a separating family
    for the category of \(\quantale Q\)-sets.
\end{prop}
\begin{proof}
    Indeed, for any pair of morphisms \(f, g:X \to Y\), 
    if \(f \not= g\) then must be some \(x \in X\) such that 
    \(f(x) \not g(x)\). Taking \(e = \extent x\) clearly separates 
    \(f\) from \(g\): \((e\in\{e\})\mapsto(x\in X)\) already suffices 
    to show they are different.
\end{proof}

\zeca{
    Salve gente! Algumas sugestões de estilo para manter a coerência do artigo:
    \begin{enumerate}
        \item Transformar essas subsessões em proposições ou algo do tipo, 
        porque não é subsessão: são construções e provas. Eu tenho colocado 
        proposição porque é a proposição “esta coisa satisfaz a propriedade 
        universal” 

        \item Separar as provas em pedaços, dizer o que cada pedaço faz, etc. 
        Eu tenho escrito begin proof[Proof: pedaço da prova] e provado 
        pedaço a pedaço. Aceito sugestões mas me pareceu razoável na hora.
    
        \item Preferir a nova notação de math mode à velha: isto é, sifrão 
        é velho e não é amigável para substituição de texto (imagine que o
        abre parênteses fosse igual ao fecha parênteses |tipo desse jeito!|
        seria bem ruim!)
    
        \item Preferir tensor a otimes, tem várias vantagens inclusive porque
        podemos mudar no futuro. Só não coloquem ele direto adjacente a 
        “[ outras coisas dentro de colchetes ]” porque ele fica bravo. O 
        correto é colocar chanves ao redor dos colchetes para evitar a ira
        dele. É um mal meio necessário.  
    
        \item Preferir amalg a coprod como operação binária, o coprod não 
        é uma operação binária e não alinha os argumentos à direita e à 
        esquerda pra ficar bonitinho.
    
        \item preferir faktor a quando quocientando por relação de equivalência
        porque fica mais bonito.
    
        \item não esquecer dos left( e dos right)
        porque fica bem horrível quando tem um bagulho enorme e uns parênteses
        minúsculos.

        \item usar o comando “set” para notação set-builder:
        set[separador] formador filtro. O parâmetro separador é opcional.
    
        \item preferir “:” depois de quantificadores, ao invés de (...)
    
        \item quebrar os aligns em múltiplos aligns conforme os blocos de 
        desigualdade vão terminando, por motivos de sanidade e também de 
        tipografia: o latex prefere não quebrar aligns no meio, então as 
        páginas ficam mais vazias e mal utilizadas com aligns longos. Vide
        a próxima página.

        \item para índices múltiplos em sups/infs/limites, pode-se usar 
            substack para fazer índices ocuparem múltiplas linhas ao invés de 
            ficarem infinitamente longos e péssimos de ler.

        \item buscar usar os comandos img, cod, etc. para domínio e codomínio. 
        Se tiverem interesse, podem ver no josealvim.sty que tem as definições 
        de muitos comandos que são de interesse.
        
        \item quebras de linha manual no modo de texto costumam indicar abominações tipográficas
    \end{enumerate}
}

\subsection{Regular monomorphisms}% in non-complete functional $\mathscr{Q}$-Sets}

A morphism is a regular monomorphism if, and only if it is a injective isometry:\\

$$\delta(x,x')=\delta(f(x),f(x'))$$

Suppose that $f:X\to Y$ is a regular monomorphism. Then exists $g,h:Y\to A$ such that $f:X\to Y$ is the equalizer of $g,h:Y\to A$. Then, $X=Eq(g,h)$ and therefore $\delta_X=\delta_Y \restriction_{X \times X}$. We can conclude that $\delta(x,x')=\delta(f(x),f(x'))$.\\

Suppose that $\delta(x,x')=\delta(f(x),f(x'))$. We can define $Y_f=((Y\coprod Y)/\sim,\delta)$, where $\sim$ is generated by $(f(x),0)\sim (f(x),1)$ and: 

\begin{align*}
\delta([(y,i)],[(y',i)])&=\delta(y,y')\\
i\neq j \Longrightarrow \delta([(y,i)],[(y',j)])&=\bigvee_{x \in X}\delta(y,f(x))\otimes \delta(f(x),y')
\end{align*}

$Y_f$ is a Q-Set. Let $i\neq j \neq k \neq i$:\\

\begin{align*}
    \delta([(y,i)],[(y',i)])&=\delta(y,y')\\
    &=\delta(y',y)\\
    &=\delta([(y',i)],[(y,i)])\\
    \\
    \delta([(y,i)],[(y',i)]) \otimes \delta([(y',i)],[(y'',i)])&=\delta(y,y') \otimes \delta(y',y'')\\
    &\leq\delta(y,y'')\\
    &=\delta([(y,i)],[(y'',i)])\\
    \\
    \delta([(y,i)],[(y',i)]) \otimes \delta([(y,i)],[(y,i)])&=\delta(y,y')\otimes \delta(y,y)\\
    &=\delta(y,y')\\
    &=\delta([(y,i)],[(y',i)])\\
\end{align*}
\begin{align*}
    \delta([(y,i)],[(y',j)])&=\bigvee_{x \in X}\delta(y,f(x))\otimes \delta(f(x),y')\\
    &=\bigvee_{x \in X}\delta(y',f(x))\otimes \delta(f(x),y)\\\\
    &=\delta([(y',j)],[(y,i)])\\
    \\
    \delta([(y,i)],[(y',j)]) \otimes \delta([(y',j)],[(y'',j)])&=\bigvee_{x \in X} \delta(y,f(x)) \otimes \delta(f(x),y') \otimes \delta(y',y'')\\
    &\leq \bigvee_{x \in X} \delta(y,f(x)) \otimes \delta(f(x),y'1)\\
    &=\delta([(y,i)],[(y'',j)])\\
    \\
    \delta([(y,i)],[(y',j)]) \otimes \delta([(y',j)],[(y'',k)])&=\bigvee_{x \in X}\bigvee_{x' \in X} \delta(y,f(x)) \otimes \delta(f(x),y') \otimes \delta(y',f(x'))\otimes \delta(f(x'),y'')\\
    &\leq\bigvee_{x \in X}\bigvee_{x' \in X} \delta(y,f(x)) \otimes \delta(f(x),f(x')) \otimes\delta(f(x'),y'')\\
    &=\bigvee_{x \in X}\delta(y,f(x)) \otimes\delta(f(x),y'')\\
    &=\delta([(y,i)],[(y'',k)])\\
\end{align*}

Define $g_0,g_1:Y \to Y_f$ as $g_i(y)=(y,i)$. Both are morphisms:\\

$$\delta(g_i(y),g_i(y'))=\delta((y,i),(y',i))=\delta(y,y')$$

The equalizer of $g_0$ and $g_1$ are precisely $Im f$:\\

\begin{align*}
g_0(y)=g_1(y) &\Longrightarrow [(y,0)]=[(y,1)]\\
&\Longrightarrow y \in Im f
\end{align*}

Thus, $f$ is regular.

\subsection{Classifier for regular monos}

Let $\Omega=(\top\coprod\top,\delta)$ where:\\

$$\delta((e,i),(e',j))=
\begin{cases}
e\otimes e', \text{ if }i=j\\
\bot, \text{ if } i\neq j
\end{cases}.$$

For each regular monomorphism $f:X \to Y$, we define $\chi_f:Y\to \Omega$ as $\chi_f(y)=(Ey,1)$. Then 


\begin{example}[Regular Subobject Classifier for Incomplete \(\quantale Q\)-Sets]
    Consider \(\Omega = \top\amalg\top\) with \(\delta\) given 
    naturally: if \(e,e'\) are in the same component, then 
    \(\delta(e,e') = e\wedge e'\), otherwise, it is \(\bot\).
    We claim, yet leave to be proven in
    \cite{AMM2023constructions}, that the above actually defines 
    \(\quantale Q\)-set by showing that it in fact is a coproduct.

    This is rather straightforward, but we have two canonical 
    arrows from a given \(X\) to \(\Omega\): \(!_l\) and \(!_r\),
    corresponding to the composition with the terminal arrow 
    and the respective inclusions into the coproduct.    

    \zeca{Como prova?} 
\end{example}
